Predictive Querying for Autoregressive Neural Sequence Models

In reasoning about sequential events it is natural to pose probabilistic queries such as "when will event A occur next" or "what is the probability of A occurring before B", with applications in areas such as user modeling, medicine, and finance. However, with machine learning shifting towards neural autoregressive models such as RNNs and transformers, probabilistic querying has been largely restricted to simple cases such as next-event prediction. This is in part due to the fact that future querying involves marginalization over large path spaces, which is not straightforward to do efficiently in such models. In this paper we introduce a general typology for predictive queries in neural autoregressive sequence models and show that such queries can be systematically represented by sets of elementary building blocks. We leverage this typology to develop new query estimation methods based on beam search, importance sampling, and hybrids. Across four large-scale sequence datasets from different application domains, as well as for the GPT-2 language model, we demonstrate the ability to make query answering tractable for arbitrary queries in exponentially-large predictive path-spaces, and find clear differences in cost-accuracy tradeoffs between search and sampling methods.

==> Sections/Appendices/query2_is_ablation.tex <==
\section{Ablation: Importance Sampling Fidelity for Long Queries}
\label{sec:is_fidelity_long_seq}



\begin{table}[H]
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      \multicolumn{8}{c}{Query Sequence Length} \\
\midrule
\# Samples &      2   &      5   &      10  &      20  &      40  &      60  &      80  &      100 \\
\midrule
10    &  0.07777 &  0.10246 &  0.11593 &  0.11698 &  0.09802 &  0.10201 &  0.10335 &  0.10958 \\
30    &  0.02963 &  0.03947 &  0.04612 &  0.04419 &  0.03933 &  0.04088 &  0.04357 &  0.04604 \\
50    &  0.01701 &  0.02458 &  0.02832 &  0.02875 &  0.02656 &  0.02607 &  0.02937 &  0.03147 \\
100   &  0.00864 &  0.01296 &  0.01521 &  0.01467 &  0.01421 &  0.01600 &  0.01823 &  0.01995 \\
300   &  0.00325 &  0.00476 &  0.00534 &  0.00510 &  0.00563 &  0.00640 &  0.00777 &  0.00799 \\
500   &  0.00183 &  0.00288 &  0.00325 &  0.00303 &  0.00360 &  0.00422 &  0.00514 &  0.00551 \\
1000  &  0.00092 &  0.00140 &  0.00167 &  0.00162 &  0.00205 &  0.00229 &  0.00282 &  0.00303 \\
3000  &  0.00030 &  0.00047 &  0.00054 &  0.00058 &  0.00076 &  0.00094 &  0.00100 &  0.00111 \\
5000  &  0.00016 &  0.00027 &  0.00033 &  0.00035 &  0.00048 &  0.00056 &  0.00060 &  0.00068 \\
10000 &  0.00009 &  0.00014 &  0.00016 &  0.00017 &  0.00025 &  0.00028 &  0.00029 &  0.00035 \\
\bottomrule
\end{tabular}
\caption{Average KL Divergence (relative entropy) between pseudo-ground truth and importance sampling estimates for 100 queries taken from \textbf{Reviews} dataset. PGT was collected with an error tolerance of $\delta = 1e^{-7}$ and a maximum sample budget of $250,000$.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      \multicolumn{8}{c}{Query Sequence Length} \\
\midrule
\# Samples &      2   &      5   &      10  &      20  &      40  &      60  &      80  &      100 \\
\midrule
10    &  0.24636 &  0.39938 &  0.49633 &  0.53261 &  0.50930 &  0.54033 &  0.54350 &  0.53290 \\
30    &  0.09374 &  0.16453 &  0.22747 &  0.23334 &  0.23325 &  0.24949 &  0.23519 &  0.23596 \\
50    &  0.06239 &  0.10865 &  0.14975 &  0.15478 &  0.16468 &  0.16498 &  0.15555 &  0.15791 \\
100   &  0.03151 &  0.05687 &  0.08451 &  0.09082 &  0.09006 &  0.09358 &  0.08501 &  0.08865 \\
300   &  0.00990 &  0.01970 &  0.03045 &  0.03279 &  0.03370 &  0.03335 &  0.03348 &  0.03332 \\
500   &  0.00598 &  0.01211 &  0.01817 &  0.02051 &  0.02115 &  0.02048 &  0.02005 &  0.02090 \\
1000  &  0.00311 &  0.00619 &  0.00953 &  0.01038 &  0.01092 &  0.01040 &  0.01036 &  0.01075 \\
3000  &  0.00105 &  0.00214 &  0.00317 &  0.00369 &  0.00358 &  0.00369 &  0.00373 &  0.00362 \\
5000  &  0.00064 &  0.00129 &  0.00197 &  0.00222 &  0.00220 &  0.00219 &  0.00224 &  0.00215 \\
10000 &  0.00033 &  0.00063 &  0.00098 &  0.00109 &  0.00110 &  0.00108 &  0.00110 &  0.00106 \\
\bottomrule
\end{tabular}
\caption{Average KL Divergence (relative entropy) between pseudo-ground truth and importance sampling estimates for 100 queries taken from \textbf{Shakespeare} dataset. PGT was collected with an error tolerance of $\delta = 1e^{-7}$ and a maximum sample budget of $250,000$.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      \multicolumn{8}{c}{Query Sequence Length} \\
\midrule
\# Samples &      2   &      5   &      10  &      20  &      40  &      60  &      80  &      100 \\
\midrule
10    &  0.19327 &  0.37587 &  0.59260 &  0.80115 &  0.98514 &  1.09345 &  1.10783 &  1.17955 \\
30    &  0.09654 &  0.18376 &  0.28232 &  0.39400 &  0.50090 &  0.55637 &  0.55334 &  0.57453 \\
50    &  0.06370 &  0.12720 &  0.19311 &  0.26374 &  0.33748 &  0.36861 &  0.37852 &  0.39491 \\
100   &  0.03546 &  0.07182 &  0.10772 &  0.14772 &  0.18664 &  0.21176 &  0.21936 &  0.22095 \\
300   &  0.01424 &  0.02773 &  0.04329 &  0.05690 &  0.07304 &  0.07871 &  0.07949 &  0.07913 \\
500   &  0.00893 &  0.01808 &  0.02747 &  0.03640 &  0.04588 &  0.04835 &  0.04881 &  0.04880 \\
1000  &  0.00503 &  0.01018 &  0.01519 &  0.01939 &  0.02337 &  0.02429 &  0.02431 &  0.02450 \\
3000  &  0.00177 &  0.00372 &  0.00543 &  0.00687 &  0.00776 &  0.00820 &  0.00800 &  0.00811 \\
5000  &  0.00114 &  0.00232 &  0.00337 &  0.00426 &  0.00478 &  0.00492 &  0.00481 &  0.00479 \\
10000 &  0.00057 &  0.00118 &  0.00173 &  0.00212 &  0.00232 &  0.00238 &  0.00234 &  0.00236 \\
\bottomrule
\end{tabular}
\caption{Average KL Divergence (relative entropy) between pseudo-ground truth and importance sampling estimates for 100 queries taken from \textbf{MOOCs} dataset. PGT was collected with an error tolerance of $\delta = 1e^{-7}$ and a maximum sample budget of $250,000$.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\begin{tabular}{lrrrrrrrr}
\toprule
{} &      \multicolumn{8}{c}{Query Sequence Length} \\
\midrule
\# Samples &      2   &      5   &      10  &      20  &      40  &      60  &      80  &      100 \\
\midrule
10    &  0.15687 &  0.27931 &  0.42376 &  0.55078 &  0.66539 &  0.74295 &  0.80917 &  0.92614 \\
30    &  0.09915 &  0.16555 &  0.24863 &  0.30317 &  0.37719 &  0.42402 &  0.43524 &  0.48099 \\
50    &  0.07670 &  0.12103 &  0.17425 &  0.21881 &  0.26294 &  0.30259 &  0.31926 &  0.33962 \\
100   &  0.05122 &  0.08178 &  0.11541 &  0.13693 &  0.16299 &  0.18352 &  0.19909 &  0.21223 \\
300   &  0.02402 &  0.03915 &  0.05160 &  0.06097 &  0.07237 &  0.08005 &  0.08406 &  0.09038 \\
500   &  0.01683 &  0.02707 &  0.03383 &  0.04074 &  0.04713 &  0.05202 &  0.05514 &  0.05796 \\
1000  &  0.00988 &  0.01540 &  0.01941 &  0.02236 &  0.02558 &  0.02821 &  0.03003 &  0.03123 \\
3000  &  0.00389 &  0.00579 &  0.00715 &  0.00832 &  0.00950 &  0.01043 &  0.01074 &  0.01122 \\
5000  &  0.00244 &  0.00357 &  0.00445 &  0.00513 &  0.00591 &  0.00641 &  0.00652 &  0.00699 \\
10000 &  0.00124 &  0.00187 &  0.00224 &  0.00261 &  0.00300 &  0.00323 &  0.00336 &  0.00356 \\
\bottomrule
\end{tabular}
\caption{Average KL Divergence (relative entropy) between pseudo-ground truth and importance sampling estimates for 100 queries taken from \textbf{Apps} dataset. PGT was collected with an error tolerance of $\delta = 1e^{-7}$ and a maximum sample budget of $250,000$.}
\end{table}

==> Sections/acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:acknowledgements}

This was was funded by ...

Alex Boyd was also funded by ...

In addition, Sam Showalter was also funded by ...

==> Sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerYes{See Section \ref{sec:discussion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We mention computational resources, PII considerations, and other ethical factors in our paper directly.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:queries}, \ref{sec:methods}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Included in supplement as a .zip file}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerNo{We gather data for multiple query histories and report median results for a given experimental setting.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
         \answerYes{See Section \ref{sec:experiments}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite all public datasets utilized.}
  \item Did you mention the license of the assets?
    \answerYes{Datasets used are all publicly available and the specific license is noted in the Appendix for each.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Datasets are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section \ref{sec:experiments}.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> Sections/conclusion.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}
 
 
TBD (can keep it short)

==> Tables/performance_4datasets.tex <==
\begin{table}[]
\begin{tabular}{ccccc}\cline{1-1}
\toprule
{} &        Amazon &         Shakespeare &          Apps &         MOOCs \\
\midrule
$|\mathcal{V}|$ &   29 &      67 &             87 &            97 \\
\hline
\multicolumn{1}{c}{$k$} & \multicolumn{4}{c}{Beam Search / Importance Sampling / Hybrid Sampling} \\
% $k$ &   Beam Search / Importance Sampling / Hybrid Sampling \\
% Test run \\
\midrule
3  &   \textbf{ 0.00 } / 1.09 / 0.72 &   \textbf{ 0.00 } / 3.15 / 1.80 &   \textbf{ 0.00 } / 2.03 / 1.17 &   \textbf{ 0.00 } / 2.32 / 1.08 \\
4  &   5.56 / 1.26 / \textbf{ 0.90 } &   \textbf{ 0.39 } / 4.64 / 3.10 &   \textbf{ 0.10 } / 3.02 / 1.54 &   \textbf{ 0.25 } / 3.51 / 1.91 \\
\hdashline
5  &  31.59 / 1.53 / \textbf{ 1.17 } &   6.62 / 6.46 / \textbf{ 4.58 } &   \textbf{ 1.15 } / 3.54 / 2.35 &   3.52 / 4.56 / \textbf{ 2.94 } \\
6  &  53.56 / 1.53 / \textbf{ 1.31 } &  20.70 / 6.23 / \textbf{ 5.98 } &   \textbf{ 2.39 } / 5.20 / 3.96 &  11.24 / 5.10 / \textbf{ 3.70 } \\
8  &  77.08 / 1.90 / \textbf{ 1.47 } &  54.98 / 7.64 / \textbf{ 6.65 } &   4.88 / 6.85 / \textbf{ 4.83 } &  37.44 / 6.70 / \textbf{ 5.34 } \\
9  &  83.55 / 2.02 / \textbf{ 1.68 } &  69.78 / 8.15 / \textbf{ 7.28 } &   4.85 / 6.52 / \textbf{ 4.77 } &  51.38 / 7.27 / \textbf{ 6.01 } \\
10 &  88.74 / 1.91 / \textbf{ 1.82 } &  79.26 / 8.77 / \textbf{ 7.61 } &  10.16 / 9.67 / \textbf{ 6.95 } &  63.77 / 7.42 / \textbf{ 6.35 } \\
11 &  90.45 / 2.09 / \textbf{ 1.87 } &  86.80 / 8.59 / \textbf{ 8.14 } &  10.57 / 7.64 / \textbf{ 5.81 } &  74.05 / 7.64 / \textbf{ 7.62 } \\
\bottomrule
\end{tabular}
\caption{1000 samples utilized for hybrid estimate. Remaining methods held to hybrid compute budget. Metric: Median Relative AE between estimate and ground truth / PGT}
\label{table:comp_results}
\end{table}
